SCORE: Soft Label Compression-Centric Dataset Condensation via Coding Rate Optimization

Dataset Condensation (DC) aims to obtain a condensed dataset that allows models trained on the condensed dataset to achieve performance comparable to those trained on the full dataset. Recent DC approaches increasingly focus on encoding knowledge into realistic images with soft labeling, for their scalability to ImageNet-scale datasets and strong capability of cross-domain generalization. However, this strong performance comes at a substantial storage cost which could significantly exceed the storage cost of the original dataset. We argue that the three key properties to alleviate this performance-storage dilemma are informativeness, discriminativeness, and compressibility of the condensed data. Towards this end, this paper proposes a \textbf{S}oft label compression-centric dataset condensation framework using \textbf{CO}ding \textbf{R}at\textbf{E} (SCORE). SCORE formulates dataset condensation as a min-max optimization problem, which aims to balance the three key properties from an information-theoretic perspective. In particular, we theoretically demonstrate that our coding rate-inspired objective function is submodular, and its optimization naturally enforces low-rank structure in the soft label set corresponding to each condensed data. Extensive experiments on large-scale datasets, including ImageNet-1K and Tiny-ImageNet, demonstrate that SCORE outperforms existing methods in most cases. Even with 30$\times$ compression of soft labels, performance decreases by only 5.5\% and 2.7\% for ImageNet-1K with IPC 10 and 50, respectively. Code will be released upon paper acceptance.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{iccv.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/method_draft.tex <==
1. task formulation
teacher network
how to build condensed dataset
two objectives: number less, performance good
aim to select representative samples to facilitate classification.


2. existing work challenge
soft label challenge, label storage more than image -> normally low rank compression

three properties
information
discriminativeness
compress include rpca


3. a unified criteria
give overall objectives
list three terms

4. theoretical analysis
a. why use coding rate?
for compressiveness, it is low rank approximation

b. how to select?
objective is a non-trivial task. state coding rate is submodular.

c. implement for compression


==> sec/methodology_new.tex <==
\section{Critical Challenges in Dataset Distillation}
\label{sec:preliminary}

\subsection{Preliminary}
The exponential growth in dataset sizes has become an ineluctable challenge. This growth motivates dataset compression approaches to preserve essential learning characteristics. Dataset condensation (DC) addresses the fundamental challenge of condensing large-scale datasets into compact yet representative forms without significant loss of efficacy. Given an original dataset $\mathcal{T}={\{{\mathbf{x}}_{i}, {\mathbf{y}}_{i}\}}^{|\mathcal{T}|}_{i=0}$, where $\mathbf{x}{i}$ represents the $i$-th image and $\mathbf{y}{i}$ its corresponding label, DC synthesizes a compact dataset $\mathcal{S}=\{({\Tilde{\mathbf{x}}_{i}}, {\Tilde{\mathbf{y}}_{i}})\}^{|\mathcal{S}|}_{i=0}$ such that $|\mathcal{S}| \ll |\mathcal{T}|$. The primary objective of DC is to preserve the essential characteristics of $\mathcal{T}$ within the condensed dataset $\mathcal{S}$. Such preservation is measured by the performance of a model $\phi(\cdot;\theta)$ when trained on $\mathcal{S}$ compared to the performance trained on the $\mathcal{T}$. Mathematically, the optimization can be formulated as a bi-level objective:
\begin{equation}
    \label{bilevel eq}
    \underset{\mathcal{S}}{\min}\EX_{\theta}[\mathcal{L}(\mathcal{T}, \theta_{\mathcal{S}})] \text{, where }  \theta_{\mathcal{S}} = \underset{\theta}{\argmin}\mathcal{L}(\mathcal{S}, \theta).
\end{equation}

This formulation encapsulates the dual challenge of DC: not only must the condensed dataset be compact, but it also enables effective model training that approaches the performance achieved with the full dataset.

\red{Merge these two sections}

\subsection{Evolution of Dataset Condensation Approaches}
The development of DC methods follow a clear trajectory. Early research focused on methods with one-hot labels using such as bi-level optimization \cite{DD} and surrogate functions \cite{zhao2021datasetcondensation, zhao2023distribution, trajectory_matching}. While these approaches demonstrated promising results on small-scale datasets, they face limitations when scaling to larger datasets, primarily due to (1) the inherent complexity of their DC algorithms, which becomes computationally intractable for large-scale datasets, and (2) the limited expressiveness of their condensed representations, especially the one-hot labels, which fail to capture the rich inter-class relationships in the original dataset.

To address these limitations, more recent approaches \cite{sre2l, rded, G-VBSM} have introduced relabeling mechanism that leverage a teacher network $\phi_{h}$ pretrained on the original dataset $\mathcal{T}$. This network generates soft labels for distilled images across training epochs $E$, resulting in a distilled dataset defined as $\mathcal{S} = \{(\Tilde{\mathbf{x}}_{i}, {\{{\Tilde{\mathbf{y}}}_{i}^{j}\}}_{j=1}^{|E|})\}$. The training process is guided by minimizing the divergence between the model's predictions and the teacher-generated soft labels:
\begin{equation}
    \label{kl divergence function}
    \mathcal{L} = -\sum_{i}^{|\mathcal{S}|} \sum_{e}^{|E|} \tilde{\mathbf{y}}^{e}_{i} \log \phi(\tilde{\mathbf{x}}^{e}_{i}; \theta),
\end{equation}
where $\tilde{\mathbf{x}}^{e}_{i}$ denotes the augmented sample at epoch $e$, and $\tilde{\mathbf{y}}^{e}_{i}$ represents its corresponding soft label generated by the teacher model.

\subsection{The Storage Overhead Dilemma}
While soft labeling has significantly enhanced the effectiveness of dataset condensation when scaling to large datasets, it has brought a critical challenge: substantial storage overhead that paradoxically contradicts the fundamental objectives of DC. For a distilled dataset $\mathcal{S}$ containing $C$ classes, the storage complexity for soft labels scales as $\mathcal{O}({E}\times{IPC}\times{C}^2)$, whereas the storage requirement for distilled images follows $\mathcal{O}({IPC}\times{HW}\times{C})$, where $H$ and $W$ represent the height and width of the distilled images, respectively. The scaling storage complexity becomes problematic for large-scale datasets such as ImageNet-1k, in which case the storage requirements for soft labels can surpass those of the condensed images themselves. This overhead complicates fair evaluation within image-per-class (IPC) budget constraints, and it also compromises the scalability of dataset condensation methods, especially in applications where storage efficiency is crucial.

% \subsection{Fundamental Properties of Effective Dataset Condensation}
\begin{proposition}[Fundamental properties of effective dataset condensation]
    Based upon analysis of DC approaches and their limitations, we identify three fundamental properties that characterize effective dataset condensation:
    \begin{enumerate}
        \item \textbf{\textit{Information Richness}}: The condensed dataset must preserve and efficiently encode the essential information from the original dataset. This includes maximizing the information retention while minimizing the storage footprint.
        \item \textbf{\textit{Discriminativeness}}: The condensed representation should keep clear discriminative boundaries between classes and capture the natural variations present in the original dataset.
        \item \textbf{\textit{Compressiveness}}: The entire condensed representation, including both images and labels, must be storage-efficient. This property has been somewhat overlooked in previous works, which focus primarily on image compression while allowing label storage to grow unconstrained.
    \end{enumerate}
\end{proposition}





\section{Methodology}
\label{sec:method}
These properties are not independent but rather form an interconnected set of requirements that must be balanced in dataset condensation solutions. Toward fulfilling all the properties, this section presents our dataset condensation framework to address these three using coding rate theory \cite{coding_rate}. Our framework is presented in \red{figure}.

\noindent \textbf{Coding Rate Theory for Information Preservation.} 
\red{In the context of deep neural networks, the learning process can be viewed through the lens of information theory \cite{information_theory}. A neural network performs two key operations: feature extraction $f(x,\theta): \mathcal{X} \rightarrow \mathcal{Z}$, which maps input data $x$ to a feature representation $z$, and classification $g(z): \mathcal{Z} \rightarrow \mathcal{Y}$, which maps these features to class labels. While the information bottleneck principle \cite{information_bottle_neck} suggests that optimal learning involves simultaneously maximizing the mutual information $I(z, y)$ while minimizing $I(x, z)$, this approach can lead to reduced generalization, particularly when dealing with degenerate distributions \cite{maximal_coding_rate}.} To address these limitations, coding rate theory provides a more robust framework for analyzing feature representations. The coding rate function $\mathcal{R}(\mathbb{Z},\epsilon)$ quantifies the minimum number of bits required to encode a feature space $\mathbb{Z} = [z_1, ..., z_n] \in \mathbb{R}^{d \times n}$ within a specified distortion tolerance \cite{rate_distortion_entropy} $\epsilon$:
\begin{equation}
\label{eq:coding rate}
    \mathcal{R}(\mathbb{Z},\epsilon) = \frac{1}{2} \log \det \left(I + \frac{d}{m{\epsilon}^2} ZZ^\top\right),
\end{equation}
where $I$ is the identity matrix and $d$ is the number of dimensions of feature $z$. This formulation provides a principled way to measure and maximize the information content of our condensed feature representations.


\noindent \textbf{Enhancing Class Discriminability.} For multi-class scenarios, where features naturally cluster into distinct subspaces, we extend the coding rate theory \cite{maximal_coding_rate} to incorporate class-aware information. Given a dataset with $C$ classes, where $Z = Z_1 \cup Z_2 \cup ... \cup Z_C$, we define the class-conditional coding rate as:
\begin{equation}
    \mathcal{R}^{c}(Z, \epsilon) = \sum_{j=1}^C \frac{\text{tr}(\Pi_j)}{2n} \log \det\left(I + \frac{d}{\text{tr}(\Pi_j)\epsilon^2}Z\Pi_jZ^T\right),
\end{equation}
where $\Pi_j \in \mathbb{R}^{n \times n}$ is a diagonal matrix and the indices of samples that belong to the jth class are set to be 1, 0 otherwise. This formulation has proven effective for rank minimization \cite{logdet_rank_minimization} and clustering \cite{coding_length_classficiation, logdet_clustering, maximal_coding_rate} problems, especially when dealing with subspace-structured distributions. By minimizing this term, we encourage the sparsification of features across different classes, thereby enhancing discriminative power.


\noindent \textbf{Soft Label Compression via Consistency.} We aim to address the storage overhead of soft labels while maintaining their effectiveness. Thus, we compress the soft labels of the distilled dataset to achieve efficient storage while maintaining training accuracy with minimal sacrifice. For an image $\mathbf{x}$, the set of soft labels generated during the relabeling process is denoted as $\mathcal{Y}^x = \{ y^x_i \mid g(f(\mathcal{A}(x))), i \in \{1,...,E\} \}$, where $\mathcal{A}$ represents random augmentations.


\begin{lemma}[Coding rate function is a concave surrogate for the rank function \cite{logdet_heuristics}]
\label{lemma:coding rate low rank}
For any matrix $Z \in \mathbb{R}^{m \times n}$, coding rate function is strictly concave w.r.t. $ZZ^\top$ and provides a smooth approximation to the rank function.
\end{lemma}

We complement the objectives of DC with low-rank soft labels by minimizing their coding rate:
\begin{equation}
    \mathcal{R}_{label}(x, \epsilon) = R(Y^x, \epsilon), \text{s.t. } y^x =  g(f(\mathcal{A}(x))).
\end{equation}

By leveraging the objective, the intra-class consistency ensures the soft labels exhibits a low-rank structure. Besides, the inherent approximate low-rank nature of soft labels makes compression feasible. Motivated by the common practice in space compression using the robust principle component (RPCA) analysis \cite{RPCA}, we find the intrinsic between coding rate theory and low-rankness and perform soft label compression through RPCA.

RPCA aims to decompose the soft label matrix $M$ of a sample into a low-rank component $L$ and a sparse matrix $S$, forming a non-convex constraint problem:
\begin{equation}
    \argmin_{L, S} rank(L) + \lambda \norm{S}_{0}, \text{subject to } M = L + S,
\end{equation}
where $\norm{\cdot}_{0}$ is $\ell0$ norm. The direct minimization of matrix rank is challenging as it leads to a non-convex optimization. To make the problem tractable, we propose to relax it to its smooth concave surrogate with coding rate function. Recalling \cref{lemma:coding rate low rank}, by transforming rank reduction in RPCA into coding rate minimization, and relaxing the $\ell0$ norm objective of $S$ to $\ell1$ norm, we obtain an efficient smooth concave heuristic for the solution as such:
\begin{equation}
    \argmin_{L, S} R(L) + \lambda \norm{S}_{1}, \text{subject to } M = L + S.
\end{equation}

We adopt the Principle Component Pursuit (PCP) framework \cite{RPCA} for its empirical effectiveness. To ensure efficient convergence, we specifically leverage the augmented Lagrange multiplier (ALM) algorithm \cite{low_rank_adm, exact_alm, inexact_alm}, which transforms the constrained optimization into a series of unconstrained problems. Our optimization procedure alternates between minimizing the rank of $L$ and the sparsity of $S$. For the pursuits of both, we employ the singular value thresholding (SVT) \cite{svt_l1, svt_matrix} throughout the alternating optimization process. \red{The detailed RPCA algorithm and theoretical analysis are demonstrated in Appendix.}

\noindent\textbf{Submodular Dataset Condensation Framework.} On the recent findings \cite{rded} that suggest realism plays a crucial role in dataset distillation, especially for model generalization, we propose a submodular and realistic selection framework that jointly optimizes for information richness, discriminative power, and label compressibility.

Submodular functions defines a set of combinarotial functions $f_{sub}: 2^{\Omega} \rightarrow \mathbb{R}$ of a finite set $\Omega$ that satisfy the condition that for every subset $X \subset Y \subseteq \Omega$ and every $x \in \Omega \setminus{Y}$, it obtains that $f_{sub}(X\cup{\{x\}}) - f_{sub}(X) \geq f_{sub}(Y\cup{\{x\}}) - f_{sub}(Y)$. Submodular functions indicate the information of a set in the context of information theoretics, which have been used in subset selection methods \cite{submodular_coreset_activelearning, PRISM}.


\begin{lemma}[Coding rate function is submodular]
\label{lemma:coding rate submodular}
Given a set of features $Z$ from a teacher model $\phi_h$, coding rate function $\mathbf{R}(\mathbb{Z},\epsilon)$ satisfies the definition of submodular function, and it can measure the compactness and informativeness of features.
\end{lemma}

This submodularity property ensures that our greedy selection algorithm achieves to maximize the coding rate-based objective. The conditional gain in submodular function value when adding an element $x$ to a selected set $\mathcal{S}$ is given by:
\begin{equation}
    f_{sub}(x|\mathcal{S}) = f_{sub}(\{x\} \cup \mathcal{S}) - f_{sub}(\mathcal{S}).
\end{equation}


Our condensed dataset aims to preserve the realism of the original dataset, while maximally helping classifiers distinguish samples of different classes, preserving the information of the original dataset, and reducing the rank of soft labels. Overall, we combine our three objectives into a unified selection goal:
\begin{equation}
\label{eq:overall selection}
    % \mathcal{R}_{select}(x|\mathcal{S}) = \mathcal{R}(f(\{x\} \cup \mathcal{S}, \theta_{h}), \epsilon) - \alpha \mathcal{R}_{label}(\{x\} \cup \mathcal{S}, \epsilon) - \beta \mathcal{R}^{c}(f(x, \theta_h), \epsilon).
    \begin{split}
    \mathcal{R}_{\text{select}}(x|\mathcal{S}) = \mathcal{R}(f(\{x\} \cup \mathcal{S}, \theta_{h}), \epsilon) \\
    \quad - \alpha \mathcal{R}_{label}(x, \epsilon) - \beta \mathcal{R}^{c}(f(\{x\} \cup \mathcal{S}, \theta_h), \epsilon).
\end{split}
\end{equation}
The proof is provided in \red{appendix} and the algorithm is presented in \cref{algorithm: coding rate selection}, where we aim to select realistic samples with maximal scores w.r.t. \cref{eq:overall selection}.

\begin{algorithm}[!t]
    \caption{Maximal Coding Rate Dataset Condensation}
    \label{algorithm: coding rate selection}
    \Input{Real Dataset $\mathcal{T}$; IPC; Teacher Network $\theta_h$}
    \Output{Subset $\mathcal{X}_{\text{select}}$}
    
    $\mathcal{X}_{\text{select}} \gets \emptyset$; \\
    $\mathcal{I}_{\text{selected}} \gets \emptyset$; \\
    \WHILE{$|\mathcal{X}_{\operatorname{sub}}| < IPC * C$}{
        $\mathcal{X}^k \gets \text{Take a batch of candidate images from } \mathcal{T} \setminus \mathcal{X}_{\text{select}}$; \\
        $j* \gets \argmax_{j \notin \mathcal{I}_{\text{selected}} \& \mathcal{X}_{j} \in \mathcal{X}^{k}} \mathcal{R}_{\text{select}}(x_j | \mathcal{X}_{\text{selected}})$; \\
        $\mathbf{X}_{\text{selected}} \gets \mathbf{X}_{\text{selected}} \cup \{\mathbf{x}_{j^*}\}$; \\
        $\mathcal{I}_{\text{selected}} \gets \mathcal{I}_{\text{selected}} \cup \{j^*\}$; \\
        
        % $\mathcal{X}^c \gets \{\mathbf{x}_i \mid \mathbf{x}_i \in \mathcal{T}, y_i = c\}$ \\
        % $\mathbf{g}_{\text{global}} \gets \nabla_{\theta}\mathcal{L}^{\mathcal{X}^c}$; \\
        % $\mathbf{X}_{\text{selected}} \gets \emptyset$; \\
        % $\mathcal{I}_{\text{selected}} \gets \emptyset$; \\
        % $\mathbf{g}_{\text{residual}} \gets \mathbf{g}_{\text{global}}$; \\
    
    }
    \Return{$\mathcal{X}_{\text{select}}$}
\end{algorithm}


